Learning Stable Robotic Skills on Riemannian Manifolds

In this paper, we propose an approach to learn stable dynamical systems evolving on Riemannian manifolds. The approach leverages a data-efficient procedure to learn a diffeomorphic transformation that maps simple stable dynamical systems onto complex robotic skills. By exploiting mathematical tools from differential geometry, the method ensures that the learned skills fulfill the geometric constraints imposed by the underlying manifolds, such as unit quaternion (UQ) for orientation and symmetric positive definite (SPD) matrices for impedance, while preserving the convergence to a given target. The proposed approach is firstly tested in simulation on a public benchmark, obtained by projecting Cartesian data into UQ and SPD manifolds, and compared with existing approaches. Apart from evaluating the approach on a public benchmark, several experiments were performed on a real robot performing bottle stacking in different conditions and a drilling task in cooperation with a human operator. The evaluation shows promising results in terms of learning accuracy and task adaptation capabilities.

==> stable-DS-Riemannian (copy)/acronyms.tex <==
\newacro{vic}[VIC]{Variable Impedance Control}

\newacro{pi2}[PI\textsuperscript{2}]{Policy Improvement with Path Integrals}
\newacro{dmp}[DMP]{Dynamic Movement Primitive}
\newacro{pdmp}[PDMP]{Periodic \ac{dmp}}
\newacro{cmp}[CMP]{Compliant Movement Primitive}
\newacro{seds}[SEDS]{Stable Estimator of Dynamical Systems}
\newacro{sds}[SDS]{Stable Dynamical Systems}
\newacro{ilc}[ILC]{Iterative  Learning  Control}
\newacro{gp}[GP]{Gaussian Process}
\newacro{gpr}[GPR]{Gaussian Process Regression}
\newacro{gmm}[GMM]{Gaussian Mixture Model}
\newacro{gmr}[GMR]{Gaussian Mixture Regression}
\newacro{ppc}[PPC]{Passivity-Preservation Control}
\newacro{tpgmm}[TP-GMM]{Task-Parameterized \ac{gmm}}
\newacro{lfd}[LfD]{Learning from Demonstration}
\newacro{il}[IL]{Imitation Learning}
\newacro{wls}[WLS]{weighted least-squares}
\newacro{spd}[SPD]{Symmetric Positive Definite}
\newacro{emg}[EMG]{Electromyography}
\newacro{vil}[VIL]{Variable Impedance Learning}
\newacro{vilc}[VILC]{Variable Impedance Learning Control}
\newacro{ai}[AI]{Artificial Intelligent}
\newacro{sea}[SEA]{Series Elastic Actuation}
\newacro{dof}[DoF]{Degree of Freedom}
\newacro{vmp}[VMP]{Via-points Movement Primitive}
\newacro{lwr}[LWR]{Locally Weighted Regression}
\newacro{rl}[RL]{Reinforcement Learning}
\newacro{auv}[AUV]{Autonomous Underwater Vehicle}
\newacro{uav}[UAV]{Unmanned Areal Vehicle}
\newacro{cmaes}[CMA-ES]{Covariance Matrix Adaptation-Evolution Strategies}
\newacro{ccdmp}[CC-DMP]{Coordinate Change-\acp{dmp}}
\newacro{gpdmp}[GPDMP]{ Global Parametric Dynamic Movement Primitive}
\newacro{bbo}[BBO]{Black-Box Optimization}
\newacro{dmpbbo}[DMPBBO]{\ac{dmp} \ac{bbo}}
\newacro{ros}[ROS]{Robotic Operating System}
\newacro{cnn}[CNN]{Convolutional Neural Network}
\newacro{nn}[NN]{Neural Network}
\newacro{aedmp}[AEDMP]{AutoEncoded \ac{dmp}}
\newacro{power}[PoWER]{Policy Learning by Weighting Exploration with the Returns}
\newacro{pd}[PD]{Proportional Derivative}
\newacro{momp}[MoMP]{Mixture of Motor Primitives}
\newacro{promp}[ProMP]{Probabilistic Movement Primitives}
\newacro{hrl}[HRL]{Hierarchical \ac{rl}}
\newacro{kmp}[KMP]{Kernelized Movement Primitive}
\newacro{rbf}[RBF]{Radial Basis Function}
\newacro{rbfnn}[RBF-NN]{\ac{rbf}-\ac{nn}}
\newacro{mle}[MLE]{Maximum Likelihood Estimation}
\newacro{qpdmp}[QP-DMP]{Unit Quaternion-based Periodic \ac{dmp}}
\newacro{rmpdmp}[RMP-DMP]{Riemannian Metric-based Periodic \ac{dmp}}
\newacro{ds}[DS]{Dynamical System}
\newacro{rmp}[RMP]{Riemannian Motion Policy}
\newacro{fdm}[FDM]{Fast Diffeomorphic Matching}
\newacro{uq}[UQ]{Unit Quaternion}
\newacro{ours}[SDS-RM]{Stable Dynamical System on Riemannian Manifolds}
\newacro{cr}[CR]{Convergence Rate}
\newacro{rmse}[RMSE]{Root Mean Square Error}
\newacro{tt}[TT]{Training Time}
\newacro{ts}[TS]{Tangent Space}
\newacro{rgmm}[R-GMM]{Riemannian \ac{gmm}}
\newacro{eflow}[E-FLOW]{Euclideanizing Flows}
\newacro{iflow}[I-FLOW]{Imitation Flow}

==> stable-DS-Riemannian (copy)/figs/dataset/dataset_figure.tex <==
\begin{figure*}
    \centering 
    \vspace{-12pt}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/1_TS_GMM.pdf}\hspace{-1mm}
    \vspace{-12pt}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/2_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/3_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/4_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/5_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/6_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/7_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/8_TS_GMM.pdf}
    \vspace{-12pt}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/9_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/10_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/11_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/12_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/13_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/14_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/15_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/16_TS_GMM.pdf}
    \vspace{-12pt}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/17_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/18_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/19_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/20_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/21_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/22_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/23_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/24_TS_GMM.pdf}
    %
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/25_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/26_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/27_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/28_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/29_TS_GMM.pdf}\hspace{-1mm}
    \includegraphics[trim={148 234 132 210},clip,width=0.12\textwidth]{figs/dataset/30_TS_GMM.pdf}
    %
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/10_TS_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/10_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/11_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/11_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/12_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/12_SPD_GMM.pdf}
%    
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/13_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/13_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/14_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/14_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/15_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/15_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/16_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/16_SPD_GMM.pdf}
%    
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/17_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/17_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/18_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/18_SPD_GMM.pdf}
%		\hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/19_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/19_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/20_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/20_SPD_GMM.pdf}
%    
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/21_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/21_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/22_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/22_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/23_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/23_SPD_GMM.pdf}
%    \hfill
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/24_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/24_SPD_GMM.pdf}
%
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/25_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/25_SPD_GMM.pdf}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/26_UQ_GMM.pdf}
%    \hspace{-2mm}
%    \includegraphics[trim={144 234 117 210},clip,width=0.12\textwidth]{figs/dataset/26_SPD_GMM.pdf}
%    \hfill
%
    \caption{Qualitative results obtained on the Riemannian LASA dataset. Reproduced trajectories (brown solid lines) are obtained by applying the diffeomorphism learned with \ac{ours} on the \ac{ts} demonstrations (black dashed lines). {It is worth noticing that \ac{ts} data are in $3$D, but we choose a view angle that makes the plot similar to the original $2$D data.}}
     \label{fig:dataset_all}
\end{figure*}

==> stable-DS-Riemannian (copy)/macrosNew.tex <==

%% new Math commands
\newcommand{\bm}[1]{\boldsymbol{\mathbf{#1}}}

\newcommand{\Kpt}{{\bm{K}_t^\mathcal{P}}}
\newcommand{\Dvt}{{\bm{D}_t^\mathcal{V}}}
\newcommand{\Kot}{{\bm{K}_t^\mathcal{O}}}
\newcommand{\Dwt}{{\bm{D}_t^\mathcal{W}}}
\newcommand{\Kdemo}{{\bm{K}^{demo}}}

\newcommand{\Kp}{{\bm{K}^\mathcal{P}}}
\newcommand{\Dv}{{\bm{D}^\mathcal{V}}}
\newcommand{\Ko}{{\bm{K}^\mathcal{O}}}
\newcommand{\Dw}{{\bm{D}^\mathcal{W}}}

\newcommand{\xhat}{{\bm{\hat{x}}}}
\newcommand{\yhat}{{\bm{\hat{y}}}}
\newcommand{\fet}{{\bm{f}_t^e}}
\newcommand{\fe}{{\bm{f}^e}}
\newcommand{\tauet}{{\bm{\uptau}_t^e}}
\newcommand{\taue}{{\bm{\uptau}^e}}
\newcommand{\spd}{\bm{\mathcal{S}}_{++}^{m}}
\newcommand{\sym}{\bm{Sym}^{m}}

\newcommand{\dz}{\Dot{z}}
\newcommand{\dP}{\dot{P}}
\newcommand{\dy}{\Dot{y}}
\newcommand{\dx}{\Dot{x}}
\newcommand{\q}{\bm{q}}
\newcommand{\p}{\bm{p}}
\newcommand{\w}{\bm{w}}
\newcommand{\dq}{\bm{\Dot{q}}}
\newcommand{\LogQ}{\text{Log}^{q}}\newcommand{\LogR}{\text{Log}^{R}}
\newcommand{\LogS}{\text{Log}^{+}}
\newcommand{\ExpQ}{\text{Exp}^{q}}
\newcommand{\ExpR}{\text{Exp}^{R}}
\newcommand{\ExpS}{\text{Exp}^{+}}
\newcommand{\X}{\bm{X}}
\newcommand{\R}{\bm{R}}
\newcommand{\dR}{\bm{\Dot{R}}}
\newcommand{\muq}{\bm{\mu}_q}

\newcommand{\D}{\bm{d}}
\newcommand{\bP}{\bm{a}}
\newcommand{\bQ}{\bm{b}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\riM}{\mathcal{M}}
\newcommand{\tsPsi}{\mathcal{T}_{\boldfrak{m}}\mathcal{M}}
\newcommand{\tsHatPsi}{\mathcal{T}_{\boldfrak{a}}\mathcal{M}}
\newcommand{\LogPsiDelta}{\text{Log}_{\Psi}\left(\Delta\right)}
\newcommand{\LogHatPsi}[1]{\text{Log}_{\boldfrak{a}}\left(#1\right)}
\newcommand{\ExpHatPsi}[1]{\text{Exp}_{\boldfrak{g}}\left(#1\right)}
\newcommand{\LogHatPsiPsi}{\text{Log}_{\boldfrak{a}}\left(\boldfrak{g}\right)}
\newcommand{\LogPsi}[1]{\text{Log}_{\boldfrak{m}}\left(#1\right)}
\newcommand{\ExpPsi}[1]{\text{Exp}_{\boldfrak{m}}\left(#1\right)}
\newcommand{\ExpPsiD}{\text{Exp}_{\Psi}\left(\D\right)}
\newcommand{\LogG}{\text{Log}_{\boldfrak{g}}}
\newcommand{\Log}{\text{Log}}
\newcommand{\ExpG}{\text{Exp}_{\boldfrak{g}}}
\newcommand{\bFg}{\boldfrak{g}}
\newcommand{\bFp}{\boldfrak{a}}
\newcommand{\bFq}{\boldfrak{b}}
\newcommand{\bFm}{\boldfrak{m}}

\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\expm[1]{\text{expm}(#1)}
\newcommand\logm[1]{\text{logm}(#1)}

\newcommand\manS[1]{\mathcal{S}^{#1}}
\newcommand\manR[1]{\mathcal{R}^{#1}}
\newcommand\manSO[1]{\mathcal{SO}\left(#1\right)}
\newcommand\manSE[1]{\mathcal{SE}\left(#1\right)}

\newcommand{\boldfrak}[1]{\bm{\mathfrak{#1}}}
\newcommand\mCal[1]{\mathcal{#1}}

\newcommand{\trsp}{{^{\top}}}

%% new TODO commands
\newcommand{\TODO}[1]{\todo[inline,caption={},color=blue!30]{TODO: #1}}

\newcommand{\ToBeDeleted}[1]{\todo[inline,caption={},color=yellow!30]{\textbf{ToBeDeleted:} #1}}


\providecommand{\matt }[1]{{\color{red}#1}}
\providecommand{\fa}[1]{{\color{blue}#1}}
\providecommand{\luka}[1]{{\color{darkgreen}#1}}
\providecommand{\alk }[1]{{\color{orange}#1}}

\providecommand{\rewrite }[1]{{\color{red}#1}}
\newenvironment{rewrite2}{%
	\color{red}
}{}

\providecommand{\change }[1]{{\color{black}#1}}
\newenvironment{change2}{%
	\color{blue}
}{}

\providecommand{\atM  }[1]{\textcolor{violet}{@Matteo:~}\textcolor{gray}{#1}}
\providecommand{\atF  }[1]{\textcolor{violet}{@Fares:~}\textcolor{blue}{#1}}
\providecommand{\atL  }[1]{\textcolor{violet}{@Luka:~}\textcolor{darkgreen}{#1}}
\providecommand{\atA  }[1]{\textcolor{violet}{@Aljaz:~}\textcolor{orange}{#1}}
\providecommand{\atAll  }[1]{\textcolor{violet}{@ALL:~}\textcolor{teal}{#1}}


%% new cross-reference commands
\newcommand{\figref}[1]{Fig.~\hyperref[#1]{\ref*{#1}}}
\newcommand{\figsref}[1]{Figures~\hyperref[#1]{\ref*{#1}}}
\newcommand{\Figref}[1]{Figure~\hyperref[#1]{\ref*{#1}}}
\newcommand{\Figsref}[2]{Figures~\ref{#1}--\ref{#2}}
\newcommand{\tabref}[1]{Tab.~\hyperref[#1]{\ref*{#1}}}
\newcommand{\secref}[1]{Sec.~\hyperref[#1]{\ref*{#1}}}
\newcommand{\Secref}[1]{Section~\hyperref[#1]{\ref*{#1}}}
\newcommand{\algoref}[1]{Algorithm~\hyperref[#1]{\ref*{#1}}}
\newcommand{\subfigref}[1]{(\subref{#1})}

%% Define format of some common idioms
\newcommand{\wrt} {{wrt}~} %
\newcommand{\eg} {{e.g.,}~} %
\newcommand{\ie} {{i.e.,}~} %
\newcommand{\etc}{\textit{etc}} %
\newcommand{\etal}{\MakeLowercase{{et al.}}}

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%% Tables
\newlength{\Oldarrayrulewidth}
\newcommand{\Cline}[2]{%
  \noalign{\global\setlength{\Oldarrayrulewidth}{\arrayrulewidth}}%
  \noalign{\global\setlength{\arrayrulewidth}{#1}}\cline{#2}%
  \noalign{\global\setlength{\arrayrulewidth}{\Oldarrayrulewidth}}
}

\definecolor{darkgreen}{rgb}{0.0,0.49,0.19}

\newcommand{\python}{\texttt{Python}}
\newcommand{\cpp}{\texttt{C++}}
\newcommand{\simulink}{\texttt{Matlab Simulink}}
\newcommand{\matlab}{\texttt{Matlab}}
\newcommand{\panda}{Franka Emika Panda}

\DeclareOption{Symbol}{\let\uppi=s}
\DeclareOption{Symbolsmallscale}{\let\uppi m}
\DeclareOption{Euler}{\let\uppi=e}
\ExecuteOptions{Euler}
\ProcessOptions\relax
\DeclareFontFamily{U}{eur}{\skewchar\font'177}
\DeclareFontShape{U}{eur}{m}{n}{%
	<-6> eurm5 <6-8> eurm7 <8-> eurm10}{}
\DeclareFontShape{U}{eur}{b}{n}{%
	<-6> eurb5 <6-8> eurb7 <8-> eurb10}{}
\DeclareSymbolFont{ugrf@m}{U}{eur}{m}{n}
\SetSymbolFont{ugrf@m}{bold}{U}{eur}{b}{n}
\DeclareMathSymbol{\upomega}{\mathord}{ugrf@m}{"21}
